The Rise of the $R$-Process in the Gaia-Sausage/Enceladus Dwarf Galaxy

Neutron star mergers (NSMs) produce copious amounts of heavy r-process elements after a time delayed inspiral process. Once NSMs are present in a galaxy, r-process elements, such as Eu, are expected to significantly increase with time. Yet, there has been limited observational data in support of Eu increasing within Local Group galaxies. We have obtained high-resolution Magellan/MIKE observations of 43 metal-poor stars in the Gaia-Sausage/Enceladus tidally disrupted galaxy with $-2.5 < \rm{[Fe/H]} < -1$. For the first time, we find a clear rise in [Eu/Mg] with increasing [Mg/H] within one galaxy. We use a chemical evolution model to study how such a rise can result from the interplay of prompt and delayed r-process enrichment events. Delayed r-process sources are required to explain the rise and subsequent leveling off of [Eu/Mg] in this disrupted galaxy. However, the rise may be explained by delayed r-process sources with either short ($\sim 10$ Myr) or long ($\sim 500$ Myr) minimum delay times. Future studies on the nature of r-process sources and their enrichment processes in the GSE will require additional stars in the GSE at even lower metallicities than the present study.

==> tab01_stub.tex <==
\begin{deluxetable*}{cccccccccc}
\tablecaption{Stellar parameters, final derived chemical abundances, and observing information for 43 stars considered in this study. The uncertainties listed include statistical and systematic uncertainties.}
\label{tab:sumtab}
\tablehead{
\colhead{\Gaia\ DR3 Source ID} & \colhead{\teff} & \colhead{\logg} & \colhead{[Fe/H]} & \colhead{$\sigma_\text{[Fe/H]}$} & \colhead{[Mg~\textsc{i}/H]} & \colhead{$\sigma_\text{[Mg~\textsc{i}/H]}$} & \colhead{[Eu~\textsc{ii}/H]} & \colhead{$\sigma_\text{[Eu~\textsc{ii}/H]}$} & \colhead{[Eu~\textsc{ii}/Mg~\textsc{i}]}
}
\startdata
31707926776039680 & 4896 & 1.89 & $-$1.96 & 0.18 & $-$1.63 & 0.12 & $-$1.57 & 0.09 & 0.06 \\
1187898485610541696 & 4451 & 1.53 & $-$1.19 & 0.18 & $-$0.95 & 0.14 & $-$0.42 & 0.12 & 0.52 \\
2472646349146818816 & 4593 & 1.51 & $-$1.55 & 0.21 & $-$1.21 & 0.12 & $-$0.83 & 0.11 & 0.38 \\
2504634406573540608 & 4814 & 2.15 & $-$1.24 & 0.21 & $-$1.00 & 0.14 & $-$0.72 & 0.12 & 0.27 \\
2505065101598396416 & 4488 & 1.49 & $-$1.32 & 0.19 & $-$1.03 & 0.14 & $-$0.74 & 0.10 & 0.29 % \\
% 2538202737087917184 & 4931 & 2.49 & $-$0.88 & 0.2 & $-$0.84 & 0.14 & $-$0.46 & 0.11 & 0.38 \\
% 2543390232947773824 & 4977 & 2.31 & $-$1.28 & 0.2 & $-$1.08 & 0.13 & $-$0.81 & 0.11 & 0.28 \\
% 2558587476508131072 & 4935 & 2.36 & $-$1.31 & 0.2 & $-$1.05 & 0.14 & $-$0.61 & 0.1 & 0.44 \\
% 2566035087238555776 & 5103 & 2.27 & $-$2.38 & 0.14 & $-$2.01 & 0.11 & $-$2.48 & 0.12 & $-$0.47 \\
% 2632995998205049216 & 4431 & 1.18 & $-$1.59 & 0.22 & $-$1.32 & 0.13 & $-$1.05 & 0.1 & 0.27 \\
% 2659914516754259456 & 4725 & 1.39 & $-$2.3 & 0.17 & $-$2.05 & 0.11 & $-$1.78 & 0.08 & 0.27 \\
% 2733469542550276352 & 5276 & 2.67 & $-$2.39 & 0.13 & $-$2.1 & 0.09 & $-$2.0 & 0.08 & 0.1 \\
% 2765074076578453760 & 4505 & 1.1 & $-$1.89 & 0.24 & $-$1.48 & 0.15 & $-$1.34 & 0.11 & 0.14 \\
% 2792504520868554240 & 4401 & 0.7 & $-$2.35 & 0.21 & $-$1.73 & 0.13 & $-$2.15 & 0.11 & $-$0.41 \\
% 2810525379008979968 & 4721 & 1.84 & $-$1.17 & 0.22 & $-$0.97 & 0.14 & $-$0.41 & 0.1 & 0.56 \\
% 2811948250134539520 & 4646 & 1.73 & $-$1.11 & 0.2 & $-$0.93 & 0.13 & $-$0.69 & 0.1 & 0.24 \\
% 2911019229961694208 & 4590 & 1.14 & $-$2.23 & 0.18 & $-$1.73 & 0.13 & $-$2.01 & 0.08 & $-$0.28 \\
% 2914192523598690048 & 5126 & 2.36 & $-$2.19 & 0.14 & $-$1.91 & 0.09 & $-$1.5 & 0.08 & 0.41 \\
% 3247170789616103808 & 4804 & 1.67 & $-$2.0 & 0.18 & $-$1.67 & 0.13 & $-$1.45 & 0.09 & 0.23 \\
% 3257948717988018304 & 4989 & 2.05 & $-$2.11 & 0.15 & $-$1.9 & 0.12 & $-$1.67 & 0.09 & 0.23 \\
% 3642334203486585728 & 4215 & 1.13 & $-$0.93 & 0.18 & $-$0.79 & 0.14 & $-$0.29 & 0.13 & 0.5 \\
% 4045622011959470464 & 4598 & 1.69 & $-$1.3 & 0.2 & $-$0.96 & 0.13 & $-$0.6 & 0.13 & 0.36 \\
% 4081038754562022528 & 4253 & 1.18 & $-$1.21 & 0.18 & $-$0.98 & 0.14 & $-$0.45 & 0.13 & 0.53 \\
% 4227203402244069120 & 4220 & 1.15 & $-$1.19 & 0.17 & $-$1.0 & 0.14 & $-$0.61 & 0.13 & 0.4 \\
% 4377687545785813248 & 4367 & 1.18 & $-$1.44 & 0.19 & $-$1.03 & 0.13 & $-$1.22 & 0.1 & $-$0.18 \\
% 4420695900880776576 & 4290 & 1.25 & $-$1.19 & 0.19 & $-$0.92 & 0.16 & $-$0.68 & 0.12 & 0.24 \\
% 4675852078212908416 & 4899 & 1.79 & $-$2.26 & 0.15 & $-$1.89 & 0.11 & $-$1.73 & 0.06 & 0.15 \\
% 4750826882756774784 & 4904 & 1.87 & $-$1.87 & 0.18 & $-$1.64 & 0.15 & $-$1.54 & 0.11 & 0.1 \\
% 4757975288886077184 & 4622 & 1.07 & $-$2.52 & 0.29 & $-$2.09 & 0.19 & $-$2.9 & 0.21 & $-$0.81 \\
% 4777636927611794432 & 4793 & 1.6 & $-$2.14 & 0.17 & $-$1.85 & 0.12 & $-$1.87 & 0.08 & $-$0.02 \\
% 4780985799511960576 & 4580 & 1.2 & $-$2.06 & 0.2 & $-$1.66 & 0.14 & $-$1.55 & 0.11 & 0.11 \\
% 4786174291804662528 & 4605 & 1.19 & $-$2.16 & 0.2 & $-$1.82 & 0.13 & $-$2.01 & 0.1 & $-$0.2 \\
% 4816836269489019904 & 4732 & 1.4 & $-$2.33 & 0.17 & $-$1.86 & 0.12 & $-$1.75 & 0.1 & 0.11 \\
% 4892850490479845120 & 4953 & 2.1 & $-$1.76 & 0.18 & $-$1.46 & 0.13 & $-$1.24 & 0.1 & 0.23 \\
% 4930039787661776896 & 4895 & 1.81 & $-$2.17 & 0.16 & $-$1.82 & 0.14 & $-$1.4 & 0.11 & 0.42 \\
% 4940475493039087872 & 4756 & 1.51 & $-$2.18 & 0.18 & $-$1.79 & 0.13 & $-$2.16 & 0.08 & $-$0.37 \\
% 4953772814866348928 & 4661 & 1.21 & $-$2.4 & 0.17 & $-$2.06 & 0.11 & $-$1.96 & 0.11 & 0.1 \\
% 5152929864265512448 & 4902 & 1.97 & $-$1.79 & 0.2 & $-$1.5 & 0.14 & $-$1.34 & 0.11 & 0.16 \\
% 5208594251034223872 & 4900 & 1.8 & $-$2.24 & 0.16 & $-$1.9 & 0.12 & $-$1.89 & 0.08 & 0.0 \\
% 5221522416131163392 & 4860 & 1.78 & $-$2.04 & 0.18 & $-$1.73 & 0.12 & $-$1.8 & 0.09 & $-$0.07 \\
% 5548763464834134400 & 4811 & 1.84 & $-$1.67 & 0.21 & $-$1.42 & 0.14 & $-$1.16 & 0.11 & 0.26 \\
% 6243816407441434752 & 4463 & 1.45 & $-$1.04 & 0.2 & $-$0.9 & 0.14 & $-$0.4 & 0.13 & 0.5 \\
% 6782821815106683008 & 4816 & 1.51 & $-$2.5 & 0.15 & $-$2.12 & 0.09 & $-$2.25 & 0.09 & $-$0.13
\enddata
\tablecomments{%
The complete version of Table~\ref{tab:sumtab} is available in the online edition of the journal. 
A short version with a subset of the columns is included here to demonstrate its form and content.
The full table contains the following columns: \Gaia\ DR3 Source ID, coordinates, observing details (date, binning, exposure time, and slit size), \teff, \logg, [Fe/H], \vt, abundances ([X/H]) for Mg, Ba, Eu, and their associated uncertainties.
}
\end{deluxetable*}

